VerA: Versatile Anonymization Applicable to Clinical Facial Photographs

The demand for privacy in facial image dissemination is gaining ground internationally, echoed by the proliferation of regulations such as GDPR, DPDPA, CCPA, PIPL, and APPI. While recent advances in anonymization surpass pixelation or blur methods, additional constraints to the task pose challenges. Largely unaddressed by current anonymization methods are clinical images and pairs of before-and-after clinical images illustrating facial medical interventions, e.g., facial surgeries or dental procedures. We present VerA, the first Versatile Anonymization framework that solves two challenges in clinical applications: A) it preserves selected semantic areas (e.g., mouth region) to show medical intervention results, that is, anonymization is only applied to the areas outside the preserved area; and B) it produces anonymized images with consistent personal identity across multiple photographs, which is crucial for anonymizing photographs of the same person taken before and after a clinical intervention. We validate our results on both single and paired anonymization of clinical images through extensive quantitative and qualitative evaluation. We also demonstrate that VerA reaches the state of the art on established anonymization tasks, in terms of photorealism and de-identification.

==> FIGURES/fig_paired_regular.tex <==


\begin{figure*}
\centering
\begin{tabular}{ccccccc}
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/input/28254.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/ciagan/28254.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/fit/28254.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/dp2/28254.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/riddle/28254.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/falco/28254.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/our_paired_inplace/28254.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/input/28462.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/ciagan/28462.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/fit/28462.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/dp2/28462.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/riddle/28462.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/falco/28462.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/our_paired_inplace/28462.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \makebox[0.136\linewidth]{Input \textbf{pair}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{CIAGAN~\cite{maximov2020ciagan}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{FIT~\cite{gu2020password}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{DP2~\cite{hukkelaas2023deepprivacy2}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{RiDDLE~\cite{li2023riddle}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{FALCO~\cite{barattin2023attribute}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{Ours} \end{tabular} \hspace{-0.2cm}
\\
\end{tabular}
\vspace{-0.3cm}
\caption{Sample qualitative results of \textit{regular paired-image} anonymization, compared with the state of the art. Best viewed on screen.}
\label{fig:paired_regular}
\end{figure*}

==> FIGURES/fig_paired_semantic.tex <==


\begin{figure}
\centering
\begin{tabular}{cccc}
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/input/28090.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/our_paired_mouth/28090.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/our_paired_nose/28090.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/our_paired_eyes/28090.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/input/28492.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/our_paired_mouth/28492.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/our_paired_nose/28492.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/anon_results/our_paired_eyes/28492.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \makebox[0.245\linewidth]{Input \textbf{pair}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.245\linewidth]{Ours (mouth)} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.245\linewidth]{Ours (nose)} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.245\linewidth]{Ours (eyes)} \end{tabular} \hspace{-0.2cm}
\\
\end{tabular}
\vspace{-0.3cm}
\caption{Our \textit{clinical paired-image} anonymization preserving from left to right the mouth, nose, or eyes of the input person.}
\label{fig:paired_semantic}
\end{figure}


==> FIGURES/fig_paired_semantic_siblings.tex <==


\begin{figure}
\centering
\begin{tabular}{cccc}
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/input/_DSC0234_0.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/our_paired_mouth/_DSC0234_0.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/our_paired_nose/_DSC0234_0.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/our_paired_eyes/_DSC0234_0.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/input/_DSC0236_0.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/our_paired_mouth/_DSC0236_0.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/our_paired_nose/_DSC0236_0.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.245\linewidth]{IMAGES/siblings/our_paired_eyes/_DSC0236_0.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \makebox[0.245\linewidth]{Input \textbf{pair}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.245\linewidth]{Ours (mouth)} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.245\linewidth]{Ours (nose)} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.245\linewidth]{Ours (eyes)} \end{tabular} \hspace{-0.2cm}
\\
\end{tabular}
\vspace{-0.3cm}
\caption{Our \textit{clinical paired-image} anonymization on a pair example taken from the standardized-capture SiblingsDB~\cite{vieira2014detecting}.}
\label{fig:paired_semantic_siblings}
\end{figure}


==> FIGURES/fig_single_regular.tex <==
\begin{figure*}
\centering
\begin{tabular}{ccccccc}
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/input/28256.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/ciagan/28256.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/fit/28256.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/dp2/28256.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/riddle/28256.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/falco/28256.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/our_paired_inplace/28256.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/input/29967.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/ciagan/29967.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/fit/29967.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/dp2/29967.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/riddle/29967.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/falco/29967.jpg} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \includegraphics[width=0.136\linewidth]{IMAGES/anon_results/our_paired_inplace/29967.jpg} \end{tabular} \hspace{-0.2cm}
\\
\hspace{-0.2cm}
\begin{tabular}{c} \makebox[0.136\linewidth]{Input} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{CIAGAN~\cite{maximov2020ciagan}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{FIT~\cite{gu2020password}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{DP2~\cite{hukkelaas2023deepprivacy2}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{RiDDLE~\cite{li2023riddle}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{FALCO~\cite{barattin2023attribute}} \end{tabular} \hspace{-0.2cm}
&
\begin{tabular}{c} \makebox[0.136\linewidth]{Ours} \end{tabular} \hspace{-0.2cm}
\\
\end{tabular}
\vspace{-0.3cm}
\caption{Sample qualitative results of \textit{regular single-image} anonymization, compared with the state of the art. Best viewed on screen.}
\label{fig:single_regular}
\end{figure*}

==> FIGURES/fig_single_semantic.tex <==
\begin{figure*}
\centering
\begin{tabular}{ccccccccc}
\hspace{-0.8cm}
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/input/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/ciagan/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/fit/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/dp2/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/riddle/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/falco/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/our_paired_mouth/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/our_paired_eyes/28660.jpg} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \includegraphics[width=0.105\linewidth]{IMAGES/anon_results/our_paired_nose/28660.jpg} \end{tabular} \hspace{-0.8cm}
\\
\hspace{-0.8cm}
\begin{tabular}{c} \makebox[0.105\linewidth]{Input} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{CIAGAN~\cite{maximov2020ciagan}} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{FIT~\cite{gu2020password}} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{DP2~\cite{hukkelaas2023deepprivacy2}} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{RiDDLE~\cite{li2023riddle}} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{FALCO~\cite{barattin2023attribute}} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{Ours (mouth)} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{Ours (eyes)} \end{tabular} \hspace{-0.8cm}
&
\begin{tabular}{c} \makebox[0.105\linewidth]{Ours (nose)} \end{tabular} \hspace{-0.8cm}
\\
\end{tabular}
\caption{Semantic single image anonymization}
\label{fig:single_semantic}
\end{figure*}
